The Shifted and The Overlooked: A Task-oriented Investigation of User-GPT Interactions

Recent progress in Large Language Models (LLMs) has produced models that exhibit remarkable performance across a variety of NLP tasks. However, it remains unclear whether the existing focus of NLP research accurately captures the genuine requirements of human users. This paper provides a comprehensive analysis of the divergence between current NLP research and the needs of real-world NLP applications via a large-scale collection of user-GPT conversations. We analyze a large-scale collection of real user queries to GPT. We compare these queries against existing NLP benchmark tasks and identify a significant gap between the tasks that users frequently request from LLMs and the tasks that are commonly studied in academic research. For example, we find that tasks such as ``design'' and ``planning'' are prevalent in user interactions but are largely neglected or different from traditional NLP benchmarks. We investigate these overlooked tasks, dissect the practical challenges they pose, and provide insights toward a roadmap to make LLMs better aligned with user needs.

==> analysis_1.tex <==
% \section{How do real-world queries shift from traditional benchmarks?}\label{sec:RQ1}

% We investigate the 2,911 datasets from the Huggingface Datasets\footnote{\url{https://huggingface.co/datasets?p=0&sort=downloads}} collected by~\citet{yin2023dynosaur} as traditional NLP benchmarks for comparison.  We interpret the differences from two aspects, domain and task type.

% \paragraph{Domain shift.} We plot the top 20 most common and representative domains of ShareGPT in Figure~\ref{fig:domain}, which account for around $73\%$ of the entire set. We observe that the domain distribution in ShareGPT is quite diverse. Notably, there is a large portion of technology-related topics. Commonly seen cases involve code writing and debugging. For Huggingface datasets, we randomly select 10 samples from each dataset as an approximation, and leverage GPT to classify the corresponding domain/topics. Similar to ShareGPT, technology-related domains also share a large portion in Huggingface. However, in Huggingface, political, legal, personal life, and film altogether contribute a large portion. We further look into the data source for Huggingface. 
% We collect the information in metadata ``Dataset Card'', where detailed information of the specific dataset is introduced. For example, MRPC dataset~\cite{dolan-brockett-2005-automatically} has the statement ``a corpus of sentence pairs automatically extracted from online \textbf{news} sources''. We then use GPT to annotate the corresponding data source as an approximation. We find that the majority of datasets are from Wikipedia and news, occupying a portion of over $80\%$. The rest mainly come from ``government reports'' and ``QA forums''.
% This phenomenon calls for dataset curation specific to domains commonly seen in user queries, and the data source should also incorporate materials in multiple formats apart from Wikipedia and news.

% \paragraph{Task type shift.}

% % \begin{figure}[hbt]
% % \centering
% % \includegraphics[width=0.48\textwidth]{figures/huggingface_datasets.pdf}
% % \caption{Representative task types of and the corresponding percentage in Huggingface datasets.}
% % \label{fig:task_type}
% % \vspace*{-3mm}
% % \end{figure}

% We categorize different tasks based on metadata statistics for all the datasets from Huggingface, as shown on the right side in Figure~\ref{fig:domain}. We filter out tasks with numbers less than $10$, and the rest samples make up to $99.8\%$ of the original set. We observe that question answering and text classification are the top-2 task types in Huggingface Datasets, summing up to more than 2/3 of the whole collection. On the contrary, in ShareGPT, almost all the user queries are free-form text generations or generations in a user-required manner. 




